Roadmap: Image reconstruction in emission tomography for the era of fast Monte Carlo simulation

Quantitative image reconstruction in positron emission tomography and single photon emission computed tomography depends on how accurately the forward model describes photon emission, transport and detection. Monte Carlo simulation is the most complete model available, yet it is mostly used as an offline reference rather than inside the reconstruction. This roadmap asks what it would take to change that. The main obstacle is not only simulation time. Iterative reconstruction requires the expectation of the measured data and the gradient of the data fidelity, whereas Monte Carlo simulation produces noisy realisations of a complete acquisition. GPU implementations, variance reduction and learned surrogate models have made simulations much faster. At the same time, modern scanners acquire ever larger data sets with larger system models, and further gains in quantitative accuracy require more detailed physics. We discuss how fast Monte Carlo simulation can improve the modelling of the system response, scatter, positron range and the joint estimation of activity and attenuation, how noisy simulations can enter reconstruction algorithms, and which computing hardware makes this feasible. Monte Carlo simulation is most valuable where analytic models fail, and most practical solutions will combine both. The most immediate benefit of fast simulators is the validation and calibration of faster analytic models, together with more accurate, absolutely quantitative scatter estimates. Key open problems are the use of noisy simulations as expectations, in particular for sparse data, the computation of gradients and adjoints, the allocation of a limited simulation budget, and the use of scattered events as a source of information rather than a nuisance. Faster simulators are necessary but not sufficient, and progress requires simulators and reconstruction methods to be developed together.

==> images/fig91_hw_trends_a.tex <==
% Panel (a) of images/fig91_hw_trends.tex: scintillation pixel elements of PET scanners versus year (semilog),
% with an exponential fit. Data: images/data/pixels_dat.csv.
% Generated by images/scripts/fig91_pixel_growth.py (fit and label positions); edit the script, not this file.
% Fit: log10(n) = -120.3391 + 0.06212 * year, i.e. a factor of 1.154 per year (doubling every 4.8 years).
\begin{axis}[roadmap, ymode=log, roadmap log y, name=a,
  width=13.83cm, height=7.8cm,
  xmin=1970, xmax=2025, ymin=1e1, ymax=1e6, xticklabels={},
  ytick={1e1,1e2,1e3,1e4,1e5,1e6},
  ylabel={scintillation pixel elements},
]
  \addplot[plotblue!75!black, dashed, line width=0.6pt, domain=1972:2025, samples=2] {10^(-120.33909+0.062118*x)};
  \addplot[only marks, mark=*, mark size=1.7pt, plotblue, mark options={draw=white, line width=0.3pt}]
    table[col sep=comma, x=year, y=scint_pix_elements] {images/data/pixels_dat.csv};
  \begin{scope}[lab/.style={font=\footnotesize\plotnums, inner sep=0.5pt, text=black!85, fill=white},
    lead/.style={black!40, line width=0.3pt, shorten <=2.4pt}]
    \node[lab] (l0) at (axis cs:1972.806,14.36) {PETT II};
    \draw[lead] (axis cs:1973,24) -- (l0.north);
    \node[lab] (l1) at (axis cs:1975.711,32) {PETT I};
    \draw[lead] (axis cs:1973,32) -- (l1.west);
    \node[lab] (l2) at (axis cs:1977.054,51.58) {PETT III};
    \draw[lead] (axis cs:1974,48) -- (l2.west);
    \node[lab] (l3) at (axis cs:1978.963,96) {ECAT II};
    \draw[lead] (axis cs:1976,96) -- (l3.west);
    \node[lab] (l4) at (axis cs:1976.674,1114) {NeuroECAT};
    \draw[lead] (axis cs:1980,792) -- (l4.east);
    \node[lab] (l5) at (axis cs:1983.806,229.4) {Scanditronix PC 384-7B};
    \draw[lead] (axis cs:1984,384) -- (l5.north);
    \node[lab] (l6) at (axis cs:1987.530,364.1) {ECAT III};
    \draw[lead] (axis cs:1985,512) -- (l6.west);
    \node[lab] (l7) at (axis cs:1985.308,3538) {ECAT 953B};
    \draw[lead] (axis cs:1989,3072) -- (l7.east);
    \node[lab] (l8) at (axis cs:1985.794,5741) {ECAT ART};
    \draw[lead] (axis cs:1989,4224) -- (l8.east);
    \node[lab] (l9) at (axis cs:1993.478,5335) {ECAT 953B/31};
    \draw[lead] (axis cs:1989,6144) -- (l9.west);
    \node[lab] (l10) at (axis cs:1983.112,2048) {Scanditronix PC 2048-15B};
    \draw[lead] (axis cs:1991,2048) -- (l10.east);
    \node[lab] (l11) at (axis cs:1995.762,8803) {ECAT 951R};
    \draw[lead] (axis cs:1992,8192) -- (l11.west);
    \node[lab] (l12) at (axis cs:1977.159,1.882e+04) {Siemens ECAT Exact HR};
    \draw[lead] (axis cs:1994,18816) -- (l12.east);
    \node[lab] (l13) at (axis cs:1989.240,1.507e+04) {ECAT Exact HR+};
    \draw[lead] (axis cs:1996,18432) -- (l13.east);
    \node[lab] (l14) at (axis cs:1985.459,9216) {Siemens ECAT Accel};
    \draw[lead] (axis cs:1999,9216) -- (l14.east);
    \node[lab] (l15) at (axis cs:1992.085,847.5) {Siemens Biograph LSO};
    \draw[lead] (axis cs:2000,9216) -- (l15.east);
    \node[lab] (l16) at (axis cs:1983.687,4.128e+04) {Siemens Biograph BGO};
    \draw[lead] (axis cs:2000,18432) -- (l16.east);
    \node[lab] (l17) at (axis cs:1988.241,2.334e+04) {Siemens Hi-Rez LSO};
    \draw[lead] (axis cs:2000,23336) -- (l17.east);
    \node[lab] (l18) at (axis cs:1996.563,1.685e+05) {ECAT HRRT};
    \draw[lead] (axis cs:2000,119808) -- (l18.east);
    \node[lab] (l19) at (axis cs:1995.573,3093) {GE Discovery LS};
    \draw[lead] (axis cs:2001,12096) -- (l19.east);
    \node[lab] (l20) at (axis cs:2001.349,4.265e+04) {ADAC/Philips Allegro};
    \draw[lead] (axis cs:2001,17864) -- (l20.south);
    \node[lab] (l21) at (axis cs:1994.799,221.4) {GE Discovery ST};
    \draw[lead] (axis cs:2003,10080) -- (l21.east);
    \node[lab] (l22) at (axis cs:1996.921,1643) {Philips Gemini};
    \draw[lead] (axis cs:2003,17864) -- (l22.east);
    \node[lab] (l23) at (axis cs:1994.545,432.5) {GE Discovery STE};
    \draw[lead] (axis cs:2005,13440) -- (l23.east);
    \node[lab] (l24) at (axis cs:2005.285,136.3) {3T MR-BrainPET insert};
    \draw[lead] (axis cs:2008,27648) -- (l24.north);
    \node[lab] (l25) at (axis cs:1996.188,2.779e+05) {Siemens Biograph mCT, TruePoint};
    \draw[lead] (axis cs:2008,32448) -- (l25.east);
    \node[lab] (l26) at (axis cs:2008.806,7068) {GE Discovery 600};
    \draw[lead] (axis cs:2009,12288) -- (l26.north);
    \node[lab] (l27) at (axis cs:1990.814,7.855e+04) {Siemens Biograph mMR};
    \draw[lead] (axis cs:2010,28672) -- (l27.east);
    \node[lab] (l28) at (axis cs:2011.000,64.2) {GE Discovery 690 PET/CT};
    \draw[lead] (axis cs:2011,13824) -- (l28.north);
    \node[lab] (l29) at (axis cs:2018.969,8305) {Philips Ingenuity TF PET};
    \draw[lead] (axis cs:2011,28336) -- (l29.west);
    \node[lab] (l30) at (axis cs:2007.516,7.861e+04) {Philips Vereos};
    \draw[lead] (axis cs:2013,23040) -- (l30.east);
    \node[lab] (l31) at (axis cs:2018.906,1.483e+04) {GE Signa PET/MR};
    \draw[lead] (axis cs:2014,20160) -- (l31.west);
    \node[lab] (l32) at (axis cs:2017.000,3794) {Siemens Biograph Vision};
    \draw[lead] (axis cs:2017,60800) -- (l32.north);
    \node[lab] (l33) at (axis cs:2017.642,1505) {GE Discovery MI PET/CT};
    \draw[lead] (axis cs:2019,24480) -- (l33.north);
    \node[lab] (l34) at (axis cs:2012.474,7.672e+05) {United Imaging uExplorer};
    \draw[lead] (axis cs:2019,564480) -- (l34.east);
    \node[lab] (l35) at (axis cs:2012.510,2.432e+05) {Siemens Biograph Vision Quadra};
    \draw[lead] (axis cs:2021,243200) -- (l35.east);
    \node[lab] (l36) at (axis cs:2017.003,3.802e+04) {GE Omni Legend};
    \draw[lead] (axis cs:2022,38016) -- (l36.east);
    \node[lab] (l37) at (axis cs:2013.879,1.411e+05) {United Imaging NeuroExplorer};
    \draw[lead] (axis cs:2022,131328) -- (l37.east);
    \node[lab] (l38) at (axis cs:2010.599,828.1) {United Imaging uMI Panorama};
    \draw[lead] (axis cs:2023,97920) -- (l38.east);
    \node[lab] (l39) at (axis cs:2013.738,4.149e+05) {PennPET Explorer};
    \draw[lead] (axis cs:2023,193536) -- (l39.east);
    \node[lab] (l40) at (axis cs:2016.239,8.636e+04) {7T BrainPET insert};
    \draw[lead] (axis cs:2024,196080) -- (l40.east);
  \end{scope}
  \node[panel] at (rel axis cs:0,1) {(a)};
  \draw[plotblue!75!black, dashed, line width=0.6pt] (axis cs:1973.380,6.422e+05) -- (axis cs:1975.766,6.422e+05)
    node[right=3pt, font=\footnotesize, text=black, inner sep=0pt]
    {exponential fit: doubling every 4.8 years};
\end{axis}

